Finding and Analyzing Crash-Consistency Bugs in Persistent-Memory File Systems

We present a study of crash-consistency bugs in persistent-memory (PM) file systems and analyze their implications for file-system design and testing crash consistency. We develop FlyTrap, a framework to test PM file systems for crash-consistency bugs. FlyTrap discovered 18 new bugs across four PM file systems; the bugs have been confirmed by developers and many have been already fixed. The discovered bugs have serious consequences such as breaking the atomicity of rename or making the file system unmountable. We present a detailed study of the bugs we found and discuss some important lessons from these observations. For instance, one of our findings is that many of the bugs are due to logic errors, rather than errors in using flushes or fences; this has important applications for future work on testing PM file systems. Another key finding is that many bugs arise from attempts to improve efficiency by performing metadata updates in-place and that recovery code that deals with rebuilding in-DRAM state is a significant source of bugs. These observations have important implications for designing and testing PM file systems. Our code is available at https://github.com/utsaslab/flytrap .

==> eval2.tex <==
\section{Observations}
\label{sec-observations}

\TODO{it might make more sense to reference the number of bugs in each category, rather than listing them explicitly, since that is already in the table. Do this once the bug count is absolutely finalized and we have looked into the fallocate bug enough to know how to categorize it}

\TODO{would be good to have a quick overview of the bugs - how many were found by the fuzzer, how many by ACE, what types of consequences they have, review confirmation/fix numbers}

\begin{table*}
    \centering 
    \begin{tabular}{llp{.3\textwidth}p{.3\textwidth}l}
        \toprule
        Bug \# & File System & Consequence & Affected system calls & Type \\ \midrule
        \begin{bug} \label{bug:nova1} \end{bug} & NOVA & File system unmountable & All & Logic \\
        \begin{bug} \label{bug:nova2} \end{bug} & NOVA & File is unreadable and undeletable & {\tt mkdir, creat} & PM \\
        \begin{bug} \label{bug:nova3} \end{bug} & NOVA & File system unmountable & {\tt write, pwrite, link, unlink, rename} & Logic \\
        \begin{bug} \label{bug:nova4} \end{bug} & NOVA & Rename atomicity broken (file disappears) & {\tt rename} & Logic \\
        \begin{bug} \label{bug:nova5} \end{bug} & NOVA & Rename atomicity broken (old file still present) & {\tt rename} & Logic \\
        \begin{bug} \label{bug:nova6} \end{bug} & NOVA & Link count incremented before new file appears & {\tt link} & Logic \\ 
        \begin{bug} \label{bug:nova7} \end{bug} & NOVA & File data lost & {\tt truncate} & Logic \\ 
        \begin{bug} \label{bug:nova8} \end{bug} & NOVA & File data lost & {\tt fallocate} & Logic \\
        \begin{bug} \label{bug:nova-fortis1} \end{bug} & NOVA-Fortis & Directory unreadable, or existing file incorrectly reverts to past state & {\tt unlink, rmdir, truncate} & PM \\
        \begin{bug} \label{bug:nova-fortis2} \end{bug} & NOVA-Fortis & File is undeletable & {\tt write, pwrite, link, rename} & Logic \\
        \begin{bug} \label{bug:nova-fortis3} \end{bug} & NOVA-Fortis & User-visible error messages & {\tt truncate} & Logic \\ 
        \begin{bug} \label{bug:nova-fortis4} \end{bug} & NOVA-Fortis & File is unreadable & {\tt truncate} & Logic \\
        \begin{bug} \label{bug:pmfs1} \end{bug} & PMFS & File system unmountable & {\tt truncate} & Logic \\
        \begin{bug} \label{bug:pmfs2} \end{bug}\&\begin{bug} \label{bug:wine2} \end{bug} & PMFS\&WineFS & Write is not synchronous & {\tt write, pwrite} & PM \\
        \begin{bug} \label{bug:pmfs3} \end{bug} & PMFS & KASAN bug report & All & Logic \\
        \begin{bug} \label{bug:pmfs4} \end{bug}\&\begin{bug} \label{bug:wine3} \end{bug} & PMFS\&WineFS & File data lost & {\tt write, pwrite} & PM \\
        \begin{bug} \label{bug:wine1} \end{bug} & WineFS & File is unreadable and undeletable & All & Logic \\
        \begin{bug} \label{bug:wine4} \end{bug} & WineFS & Data write is not atomic in strict mode & {\tt write, pwrite} & Logic \\
        % \ref{bug:wine2} & WineFS & Write is not synchronous & {\tt write, pwrite} & PM \\
        % \ref{bug:wine3} & WineFS & File data lost & {\tt write, pwrite} & PM \\
        \bottomrule
    \end{tabular}
    \label{tab:bugs}
    \caption{Bugs found by \sysname, their consequences, and the system calls that they affect.}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{p{.35\textwidth}p{.35\textwidth}p{.2\textwidth}}
        \toprule 
        Observation & Implication & Associated Bugs \\ \midrule
        Many bugs arise when performing in-place updates. & Optimizations that avoid journaling or logging should be carefully examined and thoroughly tested to ensure that they don't introduce crash consistency bugs. & \ref{bug:nova4}, \ref{bug:nova5}, \ref{bug:nova6}, \ref{bug:nova7}, \ref{bug:pmfs2}, \ref{bug:wine2} \\ \midrule
        
        Recovery code that deals with rebuilding in-DRAM state is a significant source of bugs. & Testing tools should cover remounting and recovery code, and developers should perform tests that involve remounting the file system. & \ref{bug:nova1}, \ref{bug:nova3}, \ref{bug:nova7}, \ref{bug:nova8}, \ref{bug:nova-fortis3}, \ref{bug:pmfs1}, \ref{bug:pmfs3}, \ref{bug:wine1} \\ \midrule
        
        Adding complexity to make file systems more resilient to failures can introduce new bugs without adding the ability to recover from existing ones. & In order to become widely used and trusted, PM-aware file systems need testing frameworks that account for their semantics and correctness criteria. & \ref{bug:nova2}, \ref{bug:nova-fortis1}, \ref{bug:nova-fortis2}, \ref{bug:nova-fortis3}, \ref{bug:nova-fortis4} \\ \midrule
        
        Many bugs occur due to logic or design issues, not PM programming errors. & PM crash consistency testing tools should search for logic bugs as well as PM programming errors. & \ref{bug:nova1}, \ref{bug:nova3}, \ref{bug:nova4}, \ref{bug:nova5}, \ref{bug:nova6}, \ref{bug:nova7}, \ref{bug:nova8} \ref{bug:nova-fortis2}, \ref{bug:nova-fortis3}, \ref{bug:nova-fortis4}, \ref{bug:pmfs1}, \ref{bug:pmfs3}, \ref{bug:wine1}, \ref{bug:wine4} \\ \midrule
        
        Short workloads are sufficient to expose many crash consistency bugs & Systematic test case generation of a relatively low number of small workloads can expose many bugs & \ref{bug:nova1}, \ref{bug:nova2}, \ref{bug:nova3}, \ref{bug:nova5}, \ref{bug:nova6}, \ref{bug:nova-fortis1}, \ref{bug:nova-fortis2}, \ref{bug:nova-fortis3}, \ref{bug:nova-fortis4}, \ref{bug:pmfs1}, \ref{bug:pmfs2}, \ref{bug:pmfs3}, \ref{bug:pmfs4}, \ref{bug:wine1}, \ref{bug:wine2}, \ref{bug:wine3}, \ref{bug:wine4} \\ \midrule
        
        Many bugs can be exposed by only replaying a few small writes onto prior, guaranteed-persistent state & PM file system testing will find a surprising number of bugs when restricted to a small set of crash states & \ref{bug:nova3}, \ref{bug:nova4}, \ref{bug:nova5}, \ref{bug:nova6}, \ref{bug:nova-fortis2}, \ref{bug:nova-fortis3}, \ref{bug:nova-fortis4}, \ref{bug:pmfs1}, \ref{bug:pmfs2}, \ref{bug:wine1} \\ \midrule
        
        Many bugs can only be exposed by simulating crashes during system calls & Crash consistency tools for PM file systems need to inject crashes during system calls in order to find all bugs & \ref{bug:nova3}, \ref{bug:nova4}, \ref{bug:nova5}, \ref{bug:nova6}, \ref{bug:nova-fortis1}, \ref{bug:nova-fortis2}, \ref{bug:nova-fortis3}, \ref{bug:nova-fortis4}, \ref{bug:pmfs1} \ref{bug:wine1}, \ref{bug:wine4} \\
        \bottomrule
    \end{tabular}
    \label{tab:observations}
    \caption{Observations, their implications, and associated bugs found by \sysname.}
\end{table*}


\vheading{Observation 1: Many bugs arise when performing in-place updates.} \\
\vheading{Implication 1: Optimizations that avoid journaling or logging should be carefully examined and thoroughly tested to ensure that they don't introduce crash consistency bugs.}

Many applications rely on the guarantee that certain file system operations are atomic with respect to crashes. Most file systems use journaling, shadow paging, or a log structure to provide atomic operations. However, all of these approaches negatively impact the regular-case performance of the file system. For example, journaling requires all journaled writes to be written to persistent storage twice (once as part of the journal and once in the final destination). Traditional file systems on slow storage media typically avoid using these atomicity mechanisms wherever they are not absolutely necessary for performance reasons. However, this weakens the crash consistency guarantees provided by these systems.

PM file systems have different considerations when it comes to these mechanisms. Writes to PM are so fine grained that careful usage of atomicity techniques is necessary to ensure that atomicity is not violated even for operations only involving a few persistent updates. However, PM's speed makes the cost of performing extra writes to a journal less impactful than on a hard disk or solid state drive. Still, utilizing any of these mechanisms does take up time and bandwidth, and developers can obtain performance improvements by performing in-place updates instead of using transactions for atomicity.

All four file systems we tested use a journal for atomicity, but they all have mechanisms to avoid using the journal in certain situations that developers have deemed safe. Additionally, NOVA will sometimes update its per-inode log entries in place rather than adding new ones. \TODO{x} out of 18 unique bugs found by \sysname are caused by or related to these in-place updates. 

Several bugs occur because metadata is left out of journaled transactions. For example, in bug \ref{bug:nova4}, NOVA's implementation of rename deletes a dentry in-place rather than adding it to a transaction with the other operations performed by rename. If the system crashes before the transaction is committed, the renamed file will be lost entirely. Other bugs arise as a result of the added complexity of handling in-place and journaled cases separately. For example, in bug \ref{bug:pmfs2}/\ref{bug:winefs2}, PMFS and WineFS will perform data writes in-place if the destination page has already been allocated. This by itself does not violate the systems' crash consistency guarantees, but in this additional code path, there is a missing store fence that causes {\tt write()} and {\tt pwrite()} calls to not be synchronous.

%Several of these bugs occur due to added complexity of handling in-place and journaled cases separately. For example, in bugs \ref{bug:pmfs2} and \ref{bug:winefs2}, WineFS and PMFS will perform data writes in-place if the write does not require allocating a new page. This operation could be journaled, but not doing so does not violate the file systems' crash consistency guarantees, since these file systems use undo journals to roll back updates that are interrupted by a crash. However, in the code path that handles this case, there is a missing store fence that causes {\tt write()} and {\tt pwrite()} to not be synchronous, which does violate these guarantees.

To quantify the performance impact of fixing these bugs, we ran an experiment comparing a buggy version of NOVA to a version where two bugs related to journaling in the {\tt rename()} system call are fixed. These bugs were fixed by ensuring that certain metadata updates were journaled, rather than written in place. We ran several benchmarks on a Chameleon Cloud \cite{Keahey2020} node with 112 cores, 768 GB of RAM, and 3TB of Intel Optane DC Persistent Memory module. We run two microbenchmarks and one macrobenchmark. Microbenchmark 1 creates 1000 regular files and renames them each to an unused name 1000 times. Microbenchmark 2 creates 1000 regular files and renames them to an existing file name 1000 times. The macrobenchmark involves using git to check out each of the 85 tagged stable Linux kernel version in the Linux GitHub mirror. This represents a more realistic workload involving {\tt rename()} calls. We run each benchmark 5 times and use averaged runtimes to compute slowdown. The slowdown introduced in the fixed NOVA version is given in Table \ref{tab:rename_benchmarks}. Unsurprisingly, introducing extra journaling to fix these bugs causes noticeable slowdown (20-35\%) in the microbenchmarks. However, in the macrobenchmark, the slowdown is negligible (1.1\%). These results suggest that, in real world workloads, skipping in-place update optimizations and using journaling to ensure that critical functions are crash-consistent has little impact on performance.

\begin{table}
    \centering
    \begin{tabular}{lcc}
        \toprule
        Benchmark & Overall slowdown & Per-op slowdown \\ \midrule
        Microbenchmark 1 & 19\% & 20\% \\
        Microbenchmark 2 & 19\% & 34\% \\
        Macrobenchmark & 1.1\% & 1.1\% \\
        \bottomrule
    \end{tabular}
    \label{tab:rename_benchmarks}
    \caption{Slowdown caused by fixing journal-related bugs in NOVA's {\tt rename()} implementation.}
\end{table}

\vheading{Observation 2: Recovery code that deals with rebuilding in-DRAM state is a significant source of bugs.} \\
\vheading{Implication 2: Testing tools should cover remounting/recovery code, and developers should perform tests that involve remounting the file system.}

In a traditional file system, recovering from a crash primarily involves scanning on-disk structures, like journals or logs, and updating the durable state of the file system and its contents to make sure everything is consistent. While PM file systems must also perform these operations, another important part of their recovery procedures involves rebuilding in-DRAM state that was lost in the crash. Since these file systems do not use a volatile page cache, their primary memory usage comes from storing volatile metadata that may not be worth the space to store durably, that benefits from lower access latency, and that can be restored by scanning the system after a crash (e.g., the free page list or the sizes of files). Correctly rebuilding this state is crucial for a PM file system to function properly after a crash.

We found that code dealing with recovery and rebuilding DRAM state was a significant source of bugs in PM file systems. Bugs \ref{bug:nova1}, \ref{bug:nova3}, \ref{bug:nova7}, \ref{bug:nova8}, \ref{bug:pmfs1}, \ref{bug:pmfs3}, \ref{bug:wine1}, and \ref{bug:wine4} \TODO{probably} are all located in recovery code that is related to rebuilding in-DRAM state. For example, Bug \ref{bug:nova3} in NOVA occurs when trying to traverse an inode's log in certain crash states. The log must be traversed in order to reconstruct some in-DRAM state about the inode, but this bug causes the log pointers to become inconsistent in the event of a crash and prevents this. Bug \ref{bug:pmfs1} in PMFS occurs when the system crashes during a truncate operation. When truncating files, PMFS first stores information about the operation on a ``truncate list"; if the system crashes before the truncation is complete, the truncate list can be replayed and the operation can be completed. Replaying the truncate operations requires accessing PMFS's free page list, which is stored in DRAM. We discovered that the free page list is initialized \textit{after} the truncate list is replayed in recovery, so attempting to access it during the truncate recovery causes a null pointer dereference.

We also encountered several bugs related to this DRAM state rebuilding process that could impact consistency even \textit{without} a crash. This type of bug would be difficult to find without a testing tool like \sysname that focuses on checking the consistency of remounted file system images because detecting it requires comparing the state of the system before and after it is remounted. One such bug in NOVA, Bug \ref{bug:nova7}, occurs when the same file is modified via multiple file descriptors in a single program. Modifying a file in this way can cause its log entries to be created and modified out of chronological order, but the code that rebuilds the corresponding in-DRAM state always reads logs in chronological order. This can cause data loss when the workload involves truncating the file; even though the data may be present on disk, the in-DRAM size for the file is wrong, and so some of the data is not accessible. \TODO{new fallocate bug} %We also encountered a bug in which a newly-created file's size and block count values as outputted by {\tt stat} could differ before and after the file system was remounted. This occurred because file size is calculated via different code paths when a file is created and during remount, which each used a different approach. 

We also found two crash consistency bugs (Bug \ref{bug:nova1} and \ref{bug:wine1}) that occur while accessing per-CPU structures while recovering in-DRAM state. Bug \ref{bug:nova1} occurred because NOVA had a hardcoded reference to a per-CPU structure associated with the second CPU; this caused a null pointer dereference when NOVA was run on a machine with one CPU. Bug \ref{bug:wine1} occurred because WineFS failed to properly index into an array of per-CPU journals that were read during crash recovery. While per-CPU structures are not unique to PM file systems, they are widely used in these systems to improve scalability, and play an important role in recovery.

The implication here is that file system developers and testers should both be sure to include recovery and remount code paths in their testing. Some existing work on PM crash consistency testing has included checking recovery code; Yat, XFDetector, and Witcher all run recovery code as part of their testing process. As presented in their respective papers, XFDetector and Witcher both focus primarily on checking recovery code in crash states where they believe that there are likely to be specific classes of PM programming bugs. Our findings suggest that this may not be enough to find many bugs located in recovery code.

\vheading{Observation 3: Adding complexity to make file systems more resilient to failures can actually introduce new crash consistency bugs without adding ability to recover from existing ones.} \\
\vheading{Implication 3: In order to become widely used and trusted, PM-aware file systems need testing frameworks that account for their semantics and correctness criteria.}

NOVA-Fortis is an extended version of NOVA that is designed to be fault-tolerant in the event of media errors and software bugs. It consists of four modes to increase NOVA's resilience to these faults: {\tt metadata\_csum}, which replicates inodes and per-file logs and adds checksums to detect corruption; {\tt data\_csum}, which adds checksums to detect file data corruption; {\tt data\_parity}, which computes RAID-4 parity for file data; and {\tt wprotect}, which makes PM unwritable by default and requires use of CR0.WP to enable writing. While NOVA-Fortis is not explicitly designed to increase NOVA's resilience to crashes, intuitively it would seem that these features should enable NOVA-Fortis to detect and recover from crash consistency bugs that default NOVA cannot.

We tested NOVA's {\tt metadata\_csum}, {\tt data\_csum}, and {\tt data\_parity} modes. We found that NOVA-Fortis does not offer added protection against crash consistency bugs; on the contrary, NOVA-Fortis experiences all of the bugs we found in default NOVA, and we found four new crash consistency bugs that only occur in NOVA-Fortis. All four of these new bugs occur because of bugs in code that manages checksums. Three occur in {\tt metadata\_csum} mode and one occurs in {\tt data\_csum} mode. A key theme with these bugs is that modifications data and metadata are often not atomic with updates to their checksums and replicas. This can cause checksum verification to fail after a crash even if the file is in a consistent state. Three of the four bugs follow this pattern. The fourth bug occurs in crash recovery and stems from the fact that checksum verification and subsequent repair occurs on-demand when files are accessed, but rebuilding in-DRAM state happens at mount time. If a crash occurs while a file is being truncated to a smaller size, the list of free pages that is reconstructed at mount time will include the pages that were disassociated from that file during truncation. However, if checksums become inconsistent due to the crash, NOVA-Fortis may roll the inode back to its state before the truncation, causing a set of pages to be both listed as in-use by the inode and marked free by the free page list.

Finally, the added complexity of NOVA-Fortis actually introduced a bug that impacts default NOVA as well. Bug \ref{bug:nova2} occurs due to a missing cache line flush that, according to NOVA's developers, was incorrectly removed for NOVA's default mode during the development of NOVA-Fortis. 

It is not surprising that added complexity introduced new bugs, but the existence of these bugs motivate the development of new testing tools that target PM-aware file systems and can detect these types of bugs early. Since existing PM file systems are primarily research systems without the same functionality as a full production file system, more of these bugs are likely to be introduced as these file systems are developed for production.

\vheading{Observation 4: Many bugs occur due to logic or design issues, not PM programming errors.} \\\
\vheading{Implication 4: PM crash consistency testing tools should search for logic bugs as well as PM programming errors.}

Persistent memory's low-level interface and complicated semantics have been the subject of a significant recent research on crash consistency testing. PM persistency semantics are difficult to reason about and require specialized tools to systematically test, so this focus makes sense. However, our findings show that focusing on only PM programming errors will cause testing tools to miss serious bugs. In Table \ref{tab:bugs}, \TODO{this crossref gives the wrong number - why??} we categorize each bug found by \sysname as either a logic bug or a PM programming bug. Of 18 unique crash consistency bugs found by \sysname, only 4 are due to PM programming errors. Many of the most serious bugs are \textit{not} PM programming errors; for example, all three bugs that make the file systems unmountable are logic bugs. While many of the logic bugs are directly related to PM management mechanisms, they cannot be fixed by adding missing cache line flushes or store fences. They also require a higher-level understanding of the correctness criteria for the system under test than a general-purpose crash consistency tester may have; for instance, many of the bugs require knowledge of the legal states that individual files may be in after a crash.

Existing work on testing PM applications for crash consistency issues has focused primarily on finding PM programming errors and providing a general testing framework for multiple different types of PM applications. As described in their respective papers, PMTest, PMDebugger, and Jaaru all focus entirely on PM programming errors and do not have the ability to find logic bugs. Agamotto also primarily targets PM programming errors, although it can be extended to logic bugs using developer-provided bug oracles. XFDetector and Witcher target some classes of logic bugs. XFDetector looks for ``cross-failure semantic bugs" that are generally associated with modifying data outside of a transaction or with not properly handling an uncommitted transaction in recovery, and Witcher automatically detects sequences of writes to PM that should be atomic but are not. These approaches have all been successful at finding both crash consistency and performance bugs in PM applications; however, our results imply that the scope of these techniques is not sufficient to find all bugs that impact crash consistency.

\vheading{Observation 5: Short workloads were sufficient to expose many crash consistency bugs.} \\
%\vheading{Implication 5: Systematic test case generation of a relatively low number of small workloads will expose many bugs.}
\vheading{Implication 5: Using test suites of short workloads or fuzzing for a relatively short period of time can find many bugs.}

We use ACE \cite{Mohan18} to systematically generate workloads to test PM file systems with. ACE was originally developed for use with CrashMonkey, a testing tool for traditional file systems. The developers of ACE analyzed known crash consistency bugs in traditional file systems and found that most bugs can be reproduced with short workloads consisting of three or fewer core file system operations. There was no existing set of crash consistency bugs in PM file systems for similar analysis, so we did not know if this observation would hold.

Our results show that short tests can expose many bugs in PM file systems. Of the 15 unique bugs that can be found by ACE across the four tested file systems, 13 can be found using tests with \textit{only one} core system call. The other two require two core system calls (\ref{bug:nova6} in NOVA requires a {\tt rename()} followed by a {\tt link()}, and \ref{bug:pmfs2}/\ref{bug:wine2} in PMFS/WineFS require two writes to the same file). Of the three unique bugs not found by ACE tests, two (\ref{bug:pmfs4}/\ref{bug:wine3} and \ref{bug:nova8}) require two core operations, and one (\ref{bug:nova7}) requires three. 

This observation implies that a short suite of systematically generated test cases, or a relatively short period of fuzzing, can expose many bugs in PM file systems. File systems can benefit a lot by being tested with a small set of short workloads during their development, as these tests can find many serious bugs. %It is not necessary to consider long, complicated workloads in order to find serious bugs in PM file systems. \TODO{too strong?}

%Our results show that short tests can expose many bugs in PM file systems. Of the 15 unique bugs that can be found by ACE across the four tested file systems, 13 can be found using tests with \textit{only one} core system call. The other two require two core system calls (\ref{bug:nova6} requires a {\tt rename()} followed by a {\tt link()}), and \ref{bug:pmfs2} and \ref{bug:wine2} require two writes to the same file). Of the three unique bugs not found via ACE tests, one (\ref{bug:pmfs4}/\ref{bug:wine3}) only requires two {\tt write()} calls. ACE cannot find this bug because it requires the destination address of the second write to be non-8-byte-aligned, which is a case ACE does not consider. However, ACE could be extended to generate workloads of this type. The last two bugs (\ref{bug:nova7} and \ref{bug:nova8}) require 3 and 2 core operations respectively, but both require a file to be modified using multiple file descriptors, which is also a pattern not covered by ACE.

%This observation implies that a suite of short workloads can be an effective tool for finding crash consistency bugs in PM file systems. 


% \vheading{Insight 6: Many bugs can be exposed by checking only a small subset of all possible crash states.} \\
% \vheading{Implication 6: PM file system testing will find a surprising number of bugs when restricted to a small set of crash states.}
% \TODO{way too strong of a claim - either take out or make weaker}
% \TODO{could rephrase this as - many bugs are exposed by applying only small changes (64-128 bytes) on top of guaranteed persistent state. same meaning, but might be more interesting/insightful}
% \sysname's testing approach breaks metadata and small data writes up into cache line size writes, and merges large data writes into single writes. \TODO{this wording is confusing} We inject a crash just prior to each store fence. Each considered crash state is constructed by taking the guaranteed-persistent file system state that is set at the prior store fence and applying one or more of the in-flight writes. \TODO{the following sentence doesn't take into account the fact that some bugs don't require crashes during system calls} Of the 17 unique bugs found by \sysname, all but one can be exposed by only replaying a single in-flight write onto the guaranteed-persistent file system state; the last bug only requires two in-flight writes to be applied. \TODO{figure out why that bug requires 2} To confirm this, we ran ACE-generated seq1, seq2, and seq3-metadata tests and checked every crash state. Many bugs manifest in multiple crash states, some of which include more than two in-flight writes, but all of the bugs we found can be exposed with just one or two. While this is by no means a guarantee that more bugs will not be found by checking crash states with more in-flight writes, our evidence indicates that a testing approach limited to replaying 2 in-flight writes on each crash state will still be effective at finding bugs. This restriction significantly reduces the number of crash states to be checked, making the testing process much faster. \\


\vheading{Observation 6: Many bugs are exposed by replaying a few small writes onto prior, guaranteed-persistent state.} \\
\vheading{Implication 6: Many bugs can be found by only checking a small subset of all possible crash states.}

\TODO{mention here how we ran ACE with no upper bound on number of crash states to check and didn't find any new bugs}

\sysname records metadata updates and small data writes as in cache line-sized chunks, coalesces larger data writes together, and constructs crash states by replaying these recorded writes. In order to find crash consistency bugs within system calls \sysname constructs crash states by replaying subsets of in-flight writes on top of existing, guaranteed-persistent file system state. It checks crash states corresponding to smaller subsets first, increasing the number of replayed in-flight writes in each crash state until it either hits a pre-specified threshold or checks all crash states. 

13 bugs found by \sysname require injecting a crash during the execution of a system call. \TODO{explain why the other bugs are not necessary to discuss here} Of these bugs, 12 can be exposed by replaying a single cache line sized write onto the preexisting file system state. The last bug requires two writes to be applied. Many of these bugs are also present in other crash states from the same workload that are constructed by replaying more in-flight writes, but these states to not need to be checked in order to expose the bug.

This implies that many bugs can be found by focusing on checking crash states that are constructed by slightly perturbing a consistent crash state by applying a small in-flight modification. This reduces the total state of crash states to check significantly, making the testing process shorter.

\vheading{Observation 7: Many bugs can only be exposed by simulating crashes during system calls.} \\
\vheading{Implication 7: Crash consistency testing tools for PM file systems need to inject crashes during system calls in order to find all bugs.}

The current state of the art in crash consistency testing for traditional file systems has not found any crash consistency bugs by injecting crashes in the middle of file system operations. CrashMonkey \cite{Mohan18} primarily targets bugs that arise due to crashes after a persistence point (an {\tt fsync}, {\tt fdatasync}, or {\tt sync}), but does have the ability to inject crashes during system call execution and to check the resulting crash states for bugs. However, this testing did not yield any new bugs. Hydra \cite{Kim2019} only checks crashes after persistence points.

\sysname checks crash states that arise due to crashes during and after system calls. The majority of the bugs that we found - 14 out of 18 - require a crash to occur during a system call in order to be exposed. For example, \sysname found two separate bugs in NOVA that break atomicity during the {\tt rename()} system call. Both of these bugs require a crash to occur \textit{during} a {\tt rename()} call because they are caused by certain pieces of data not being included in a transaction. Only checking crash states after the rename operation completes would not expose these bugs, because by that point the relevant transactions have committed and the rename is guaranteed to be complete because NOVA's rename implementation is synchronous. Another bug in WineFS's strict mode breaks the guarantee that file data write are atomic, and also requires a simulated crash while the data is being written in order to occur.

This observation implies that crash consistency testing tools for PM file systems need inject crashes during system calls and check the resulting crash states, or they will not catch all bugs. Further, these tools must account for the crash consistency guarantees made by PM file systems, which are typically much stronger than those of traditional file systems, in order to detect many bugs.
\\

% Some weaker ideas for insights - could we turn these into anything interesting?
% \begin{enumerate}
%     \item A lot of bugs occur during truncate operations - potentially significant for memory mapped PM applications that might use truncate to create files for their persistent address space?
%     \item Many bugs impact multiple system calls - demonstrates the severity of these bugs? (or is it just because these are not well tested systems)
%     \item More store fences make it a LOT easier to test PM systems - way fewer crash states. While being more liberal with store fences would impact performance it will not introduce new bugs (since adding a store fence just constrains the write ordering to a subset of what was already possible) and makes things easier to test.
%     \item Systems like NOVA, PMFS, WineFS are MUCH easier to test than asychronous file systems like ext4 dax because they are synchronous, have relatively few in flight writes, etc. 
% \end{enumerate}

% \begin{figure}
% \pgfplotsset{scaled y ticks=false}
% \plot{results/TimeToFindBugs.csv}{}
% \caption{Cumulative time taken to find the crash consistency bugs.} 
% \end{figure}

% \subsection{Limitations}

% As our approach relies on a handwritten logging module, mistakes in this logger can cause false positives or cause bugs to be accidentally missed if there are mistakes in how the logger re-implements the operation it is recording. We ran into this issue several times during the development of the tool. An early version of our first set of loggers did not correctly ensure that flushed cache lines were actually cache-line-aligned, resulting in several false positive bugs. We later discovered that our understanding of the underlying implementation of NOVA, PMFS, and WineFS's non-temporal memcpy function was incorrect, and that it included a store fence that was not explicitly described in its documentation. This mistake also resulted in two false positive bugs, both of which were believed to be a missing store fence after a non-temporal store. We rescinded several of these bug reports before they were considered by developers, but interestingly, several of the false positives were actually confirmed and ``fixed" before we realized that they were incorrect. This experience goes to show how difficult it is to apply the semantics of persistent memory to real code and to understand where things can go wrong. 

% In general, our approach can produce false positives if there are bugs in the logger module or the testing infrastructure. We used our Syzkaller-based fuzzer to test our testing infrastructure as well as the file systems themselves and to find bugs that caused false positives. This approach is also limited by the test workloads it is provided and by the checks it performs on the file system, and will not find every crash consistency bug in a tested file system.

==> related.tex <==
\section{Related work}
\label{sec-related}

\subsection{Crash consistency testing in non-PM file systems}

As all file systems are difficult to test for crash consistency bugs, there are many tools and approaches aimed at ensuring that traditional file systems are crash safe. CrashMonkey \cite{Mohan18} is a black box record-and-replay framework that logs writes made to disk by a file system and reconstructs crash states to test based on these writes. Hydra \cite{Kim2019} and Janus \cite{Xu2019} are recent file system fuzzers. Janus focuses on memory errors in traditional file systems, while Hydra also checks for crash consistency bugs and programming errors like specification violations. eXplode \cite{Yang2006} and FiSC \cite{Yang2004} are file system model checking tools that target both crash consistency bugs and bugs in regular execution. Both model checkers require modifications to the operating system kernel and/or the file system to log file system data and explore states.

Recent work has also explored building verified storage systems with provable crash consistency guarantees. FSCQ \cite{Chen2015, Chen2017}, BilbyFS \cite{Amani2016}, Yxv6 \cite{Sigurbjarnarson2016}, and VeriBetrKV \cite{Hance2020} are formally-verified file and storage systems that are guaranteed to be free of crash consistency bugs. All of this work has focused on building new verified storage systems from scratch and cannot be used to verify existing systems written in C. To the best of our knowledge, there are no formally verified persistent memory file systems.

\subsection{Persistent memory crash testing}

The difficulty of managing persistent data on PM has also led to a number of tools for testing programs for persistent memory. Most of this work has focused primarily on memory-mapped PM applications, in which an application maps a region of persistent memory directly into its address space using {\tt mmap()}. 

Yat \cite{Lantz2014} and PMTest \cite{Liu2019} are the only two PM crash consistency testing tools that have been used on PM file systems. Yat was built specifically for PMFS, although it can be used to test other types of PM programs as well. Yat uses a hypervisor-based recording technique to log all writes to PM and reconstructs crash states to check. It produces an extremely large number of crash states; one of the three reported test workloads used with PMFS would over five years to run fully. Yat is not open source, and the exact set of bugs it found is not available. PMTest focuses specifically on a class of crash consistency bugs that we refer to as PM programming errors. These bugs are caused by missing cache line flushes or missing store fences. PMTest also looks for performance bugs caused by extra cache line flushes or store fences that are not required for crash consistency. PMTest found one performance bug in PMFS, but no crash consistency bugs.

PMTest and its successor, XFDetector \cite{Liu2020} both require source code to be annotated to indicate when data should become persistent or to mark regions of interest for testing. XFDetector looks for ``cross-failure" bugs that involve recovery code as well as regular execution code. Pmemcheck \cite{pmemcheck} is a Valgrind-based tool that also requires code to be instrumented, although Intel's PMDK libraries \cite{pmdk} are already instrumented for use with Pmemcheck. PMFuzz \cite{Liu2021} is a fuzzer designed to generate test workloads and images to be used by another testing tool like XFDetector or Pmemcheck. PMDebugger \cite{Di2021}, which proposes a set of data structures and debugging rules to speed up checking, requires some source code annotation as well.

Agamotto \cite{Neal20}, a symbolic executor built on KLEE, does not require manual annotation of source code and focuses on finding PM programming errors and performance bugs. Witcher \cite{Fu2021} is a tool for testing PM key-value stores that also does not require source code annotation. Witcher looks for both PM programming errors as well as ``persistence atomicity violations" where multiple updates that are intended to be atomic may be split up by a crash. Jaaru \cite{Gojiara2021} is a model checker for PM applications that focuses on detecting bugs related to memory stores that commit transactions to reduce the number of crash states to check. None of these tools were used to test PM file systems.

% Yat \cite{Lantz2014} is the only PM testing framework aimed specifically at testing file systems. It was designed specifically for PMFS, although it could hypothetically be applied to other PM programs and file systems. Like \sysname, Yat uses a record-and-replay approach to create and check crash states. Unlike \sysname, their approach relies on a hypervisor-based recording technique that forces a VM exit on each PM-related instruction. Yat also produces an extremely large number of crash states; of three test workloads that they report using, one containing a mix of 1200 commands to create files and directories and write small amounts of code would take over 5 years to test fully. Yat is not open source, and the exact set of bugs it found is not provided. 

% Pmemcheck \cite{pmemcheck} is a Valgrind-based tool developed by Intel to find bugs in persistent memory programs. PMDK is already instrumented for use with Pmemcheck. Pmemcheck is able to detect PM programming errors, performance bugs, and situations in which the same memory is added to two concurrent transactions. Pmemcheck cannot be used with kernel code.

% PMTest \cite{Liu2019} is a testing tool that focuses specifically on a class of crash consistency bugs that we refer to as PM programming errors. PM programming errors arise as a result of missing cache line flushes or store fences. PMTest also looks for performance bugs, in which the program contains extra cache line flushes or store fences that are not necessary for crash consistency. PMTest requires the source code of the program being tested to be annotated to indicate the correct ordering of writes and the point at which data should become persistent, which is not significantly different from adding cache line flushes and store fences in the first place. PMTest can also not detect higher-level logic bugs. PMTest was applied to one persistent memory file system (PMFS), but found no crash consistency bugs. 

% XFDetector \cite{Liu2020} is follow-up work to PMTest, and adds support for finding bugs that may only be exposed by considering both code that runs before and after a crash. In addition to detecting PM programming errors, XFDetector also looks for ``cross-failure semantic bugs," in which bugs in the design or implementation of crash recovery mechanisms result in crash consistency issues. XFDetector requires developers to annotate source code to indicate which code regions to check for crash consistency bugs. XFDetector uses a tracing mechanisms that can only be applied to user space code, and it was not used to check any persistent memory file systems.

% PMFuzz \cite{Liu2021} is a fuzzer built on AFL++ aimed at persistent memory applications. It mutates both program inputs and the PM image to find inputs to PM programs that achieve high code coverage, and uses XFDetector and Pmemcheck to detect bugs. PMFuzz runs in user space and was not used to test any file systems.

% Agamotto \cite{Neal20} is a symbolic execution engine targeted at finding PM programming errors in memory-mapped PM applications. Like PMTest, Agamotto looks for both crash consistency bugs and performance bugs. Finding other classes of bugs requires custom, developer-provided oracles. Agamotto is built on KLEE, which does not dive into kernel code and thus cannot be used to test most persistent memory file systems. 

% Witcher \cite{Fu2021} is a tool that looks for PM programming errors,  ``persistence atomicity violations" in which assumptions about the atomcity of sequences of write are violated, and performance bugs. Witcher avoids requiring source code annotation by statically inferring ``likely-correctness conditions" from source code. It determines whether the likely-correctness conditions hold by comparing outputs from crashing executions to outputs from non-crashing executions, which is similar to the consistency checking approach we use for \sysname. Witcher focuses on checking PM key-value stores, and was not used to test PM file systems. 

==> tbl-ace-runtime.tex <==
\begin{table}  
    \centering
    \begin{tabular}{llrr}
        \toprule 
        Seq length & File system & Time & Crash states \\ \midrule
        \multirow{4}{*}{seq-1} & NOVA & 8 & 2777 \\
                                & NOVA-Fortis & 11 & 4717 \\
                                & PMFS & 10 & 6706 \\
                                & WineFS & 9 & 2224 \\ \midrule
        \multirow{4}{*}{seq-2} & NOVA & 453 & 159360 \\
                                & NOVA-Fortis & 655 & 255407 \\
                                & PMFS & 567 & 369603 \\
                                & WineFS & 542 & 127355 \\ \midrule
        \multirow{3}{*}{seq-3 metadata} & NOVA & 997 & 3711529 \\
                                & NOVA-Fortis & 1580 & 5416178 \\
                                & PMFS & 1620 & 9936313 \\
        \bottomrule
    \end{tabular}
    \caption{Run time in minutes and number of crash states tested with ACE tests on different file systems.}
    \label{tab:acetests}
\end{table}


==> tbl-fuzzer.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lrr}
        \toprule
        File system & Crash states tested & Workloads/min \\ \midrule
        NOVA & 3911480 & 105 \\ 
        NOVA-Fortis & 6004304 & 92 \\
        PMFS & 27749007 & 182 \\ 
        WineFS & 3486986 & 111 \\
        \bottomrule
    \end{tabular}
    \caption{Crash states and tests after running fuzzer for 18 hours on 15 VMs}
    \label{tab:fuzzer_runs}
\end{table}


==> workloads.tex <==
\section{Workload Generation}
\label{sec-workloads}

We used two approaches, systematic generation and fuzzing, to generate workloads for our testing infrastructure. This section describes these two approaches.

\subsection{ACE workloads}

The first workload generation approach we used is based on the Automatic Crash Explorer (ACE) tool from the CrashMonkey project \cite{Mohan18}. ACE was built to exhaustively generate workload that fit a certain structure in order to test traditional file systems for crash consistency bugs. It focuses on short workloads with frequent {\tt fsync}, {\tt fdatasync}, or {\tt sync} calls, as these are required to obtain crash consistency guarantees in traditional file systems.

Given a sequence length $n$, ACE first generates a set of ``skeletons", each consisting of $n$ core file system operations, each corresponding to a system call. ACE exhaustively constructs all possible length-$n$ sequences from a set of predetermined file system operations. The initial skeletons leave the specific files to modify unspecified. ACE then expands the workload space again, using a predetermined set of files, by constructing all possible workloads on that set of files using each skeleton. Finally, ACE determines a set of setup operations that must be added to each workload in order to ensure that the core file system operations succeed. ACE outputs a set of workloads that are ready to run in the CrashMonkey framework that exhaustively cover a subset of the entire file system workload space. A workload with $n$ system calls is called a ``seq-$n$" workload. The original version of ACE generated 300 seq-1 workloads and 254k seq-2 workloads; they also tested subsets of the seq-3 workload set, which amounted to about 3 million workloads. 

We use a modified version of ACE to generate workloads for \sysname. First, since system calls in the {\tt fsync} family do not have the same crash-consistency significance in PM file systems as they do in traditional file systems, we remove them from our version of ACE. This significantly reduces the number of workloads generated, as we do not need to consider workloads that differ only in which of these system calls they use before a crash. The PM file systems that we test are also missing some features that the original CrashMonkey tested; for example, NOVA only supports the {\tt FALLOC\_FL\_KEEP\_SIZE} flag for the {\tt falloc} system call, and it does not support extended attributes. Removing these unsupported options from our modified version of ACE further reduces the number of workloads that it generates.

\TODO{confirm the number of workloads from each and report here}

\subsection{Syzkaller}

In addition to systematic test case generation, we also generated workloads using coverage-based grey-box fuzzing. As is standard in grey-box fuzzing, our fuzzer starts with an initial set of test cases (seeds) and uses genetic programming to generate new tests for \sysname~ from those seeds. \sysname~ executes the workloads generated by the fuzzer and reports back whether the test produced a crash consistency bug along with the edge coverage achieved by the test on the target kernel. If the test case covered new parts of the kernel, then the fuzzer adds the test to its set of seeds and generates new test cases. 

Our fuzzer implementation is based on Syzkaller \cite{syzkaller}, a state-of-the-art grey-box kernel fuzzer. At it's core, Syzkaller generates workloads by randomly selecting sequences system calls and their argument values. However, Syzkaller is able to generate interesting workloads that bypass the shallow, error handling, code of the kernel by using a detailed template. This template specifies each system call supported by the target OS along with \emph{refined} types for their arguments. For example, Syzkaller's template for {\tt open} specifies that the first argument is a string, the second argument is a {\tt open_flags} type which refines {\tt int}, the third argument is a {\tt mode_flags} type and it also returns a resource type {\tt fd} that refines {\tt int}

We made two modifications to Syzkaller to adapt it to our setting. First, we restrict Syzkaller to only generate test cases containing core file system system calls. Second, we extend Syzkaller to record the recovery code-coverage of each test in addition to the straight line code coverage. In particular, we track the code coverage achieved from mounting the crash states generated by \sysname~ for each workload. We then add that workload to Syzkaller's set of seeds if it achieved new straight line coverage or new coverage when mounting crash states. 
